On subgraph complementation to H-free graphs

For a class $\mathcal{G}$ of graphs, the problem SUBGRAPH COMPLEMENT TO $\mathcal{G}$ asks whether one can find a subset $S$ of vertices of the input graph $G$ such that complementing the subgraph induced by $S$ in $G$ results in a graph in $\mathcal{G}$. We investigate the complexity of the problem when $\mathcal{G}$ is $H$-free for $H$ being a complete graph, a star, a path, or a cycle. We obtain the following results: - When $H$ is a $K_t$ (a complete graph on $t$ vertices) for any fixed $t\geq 1$, the problem is solvable in polynomial-time. This applies even when $\mathcal{G}$ is a subclass of $K_t$-free graphs recognizable in polynomial-time, for example, the class of $(t-2)$-degenerate graphs. - When $H$ is a $K_{1,t}$ (a star graph on $t+1$ vertices), we obtain that the problem is NP-complete for every $t\geq 5$. This, along with known results, leaves only two unresolved cases - $K_{1,3}$ and $K_{1,4}$. - When $H$ is a $P_t$ (a path on $t$ vertices), we obtain that the problem is NP-complete for every $t\geq 7$, leaving behind only two unresolved cases - $P_5$ and $P_6$. - When $H$ is a $C_t$ (a cycle on $t$ vertices), we obtain that the problem is NP-complete for every $t\geq 8$, leaving behind four unresolved cases - $C_4, C_5, C_6,$ and $C_7$. Further, we prove that these hard problems do not admit subexponential-time algorithms (algorithms running in time $2^{o(|V(G)|)}$), assuming the Exponential Time Hypothesis. A simple complementation argument implies that results for $\mathcal{G}$ are applicable for $\overline{\mathcal{G}}$, thereby obtaining similar results for $H$ being the complement of a complete graph, a star, a path, or a cycle. Our results generalize two main results and resolve one open question by Fomin et al. (Algorithmica, 2020).

==> algo/p3-free.tex <==
\subsection{$P_3$}
\label{p3-free}


In this section, we obtain a polynomial-time algorithm for \SCG\ when $\mathcal{G}$ is the class of $P_3$-free graphs, i.e., every graph in $\mathcal{G}$
is a cluster graph.\sandeep{define cluster graph in preliminaries}.

Let $G$ be an instance of \SCG, where $\mathcal{G}$ is the class of cluster graphs.  
Assume that $G$ is not a trivial yes-instance, i.e., there exists an induced $P_3$ in $G$.
Further, assume that there exists a set $S\subseteq V(G)$ such that $G\oplus S$ is $P_3$-free.
Clearly, $|S|\geq 2$. Let $u,v$ be two vertices in $S$. 
With respect to $S, u, v$, we partition the set of vertices in $V(G)\setminus \{u,v\}$ into eight sets as given below.
This is depicted in Figure~...\sandeep{draw a figure}

\begin{enumerate}[(i)]
	\item $S_{uv}=S\cap N(u) \cap N(v)$
	\item $S_{\overline{uv}} = S\cap \overline {N[u]} \cap \overline{N[v]}$ \sandeep{define open/closed neighborhoods in preliminaries.}
	\item $S_{u\overline{v}}=S\cap (N(u)\setminus N[v])$ 
	\item $S_{\overline{u}v}=S\cap (N(v)\setminus N[u])$
	\item $T_{uv}=(N(u)\cap N(v))\setminus S$
	\item $T_{\overline{uv}}=(\overline{N[u]}\cap\overline{N[v]})\setminus S$
	\item $T_{u\overline{v}}=(N(u)\setminus N[v])\setminus S$
	\item $T_{\overline{u}v}=(N(v)\setminus N[u])\setminus S$
\end{enumerate}

Clearly, $S=S_{uv}\cup S_{\overline{uv}}\cup S_{u\overline{v}}\cup S_{\overline{u}v}\cup \{u,v\}$, 
and $V(G)\setminus S = T_{uv}\cup T_{\overline{uv}}\cup T_{u\overline{v}}\cup T_{\overline{u}v}$.

\begin{observation}
 \label{obs:p3-clique}
Let $G$ be a graph and $S\subseteq V(G)$ be such that $|S|\geq 2$ and $G\oplus S$ is $P_3$-free.
Assume that $S$ forms a clique in $G$. Let $u,v$ be any two vertices in $S$. 
Then $S_{\overline{uv}}, S_{u\overline{v}},S_{\overline{u}v},$ and $T_{uv}$ are empty.
\end{observation}
\begin{proof}
  The assumption that $S$ is a clique directly implies that the sets $S_{\overline{uv}}, S_{u\overline{v}},$ and $S_{\overline{u}v}$ are empty as
  either $u$ or $v$ is nonadjacent to each of them. Assume that $T_{uv}$ is nonempty and has a vertex $z$. 
  Then $\{u,v,z\}$ induces a $P_3$ in $G\oplus S$, which is a contradiction. Therefore, $T_{uv}$ is empty. 
  \sandeep{define in preliminaries what it means by nonadjacent.}
\end{proof}

\begin{observation}
 \label{obs:p3-nonclique}
 Let $G$ be a graph and $S\subseteq V(G)$ be such that $|S|\geq 2$ and $G\oplus S$ is $P_3$-free. 
 Assume that $S$ is not a clique. Let $u,v$ be two nonadjacent vertices in $S$. Then the following are true.
 \begin{enumerate}[(i)]
     \item $S_{u\overline{v}}$ and $S_{\overline{u}v}$ are empty;
     \item $S_{\overline{uv}}$ is an independent set;
     \item $T_{uv}$ is a clique;
     \item $S_{uv}$ and $T_{uv}$ are nonadjacent, and $S_{\overline{uv}}$ and $T_{\overline{uv}}$ are nonadjacent;
 \end{enumerate}
\end{observation}
\begin{proof}
  \begin{enumerate}[(i)]
      \item Assume that $S_{u\overline{v}}$ contains a vertex $z$. Then $\{u,v,z\}$ induces a $P_3$ in 
      $G\oplus S$, which is a contradiction. Therefore, $S_{u\overline{v}}$ is empty. With similar arguments, we 
      can prove that $S_{\overline{u}v}$ is empty.
      \item Assume for a contradiction that $S_{\overline{uv}}$ has two adjacent vertices $x$ and $y$.
      Then $\{x,y,u\}$ induces a $P_3$ in $G\oplus S$, which is a contradiction.
      \item Assume for a contradiction that there are two nonadjacent vertices $x$ and $y$ in $T_{uv}$.
      Then $\{x,y,u\}$ induces a $P_3$ in $G\oplus S$, which is a contradiction.
      \item We will prove that $S_{uv}$ and $T_{uv}$ are nonadjacent. Similar arguments prove that $S_{\overline{uv}}$
      and $T_{\overline{uv}}$ are nonadjacent. For a contradiction, assume that there is a vertex $x\in S_{uv}$
      and $y\in T_{uv}$ such that $x$ and $y$ are adjacent. Then $\{u,x,y\}$ induces a $P_3$ in $G\oplus S$, which is a contradiction.
  \end{enumerate}
\end{proof}


Let $\Pi$ be the property that a given graph $G$ is $P_3$-free, i.e., no induced subgraph of $G$ forms a $P_3$. Here we try to find a solution(if exists) $S\subseteq V(G)$ such that $G\oplus S$ is $P_3$-free in polynomial time. Consider $|V(G)|\geq 3$. let $u$ and $v$ be two distinct vertices in $G$. Now depending on the adjacencies of $u$ and $v$ we divide the vertex set of $G$ into eight parts.
\begin{enumerate}[(1)]
	
	\item$A=S\cap \overline {N(u)} \cap \overline{N(v)}$
	\item $B=S\cap N(u) \cap N(v)$
	\item $C=S\cap (N(u)$\textbackslash $N(v))$ 
	\item $D=S\cap (N(v)$\textbackslash $N(u))$
	\item $E=(N(u)$\textbackslash $N(v))$\textbackslash $S$
	\item $F=(N(v)$\textbackslash $N(u))$\textbackslash $S$
	\item $H=(N(u)\cap N(v))$\textbackslash $S$
	\item $J=(\overline{N(u)}\cap\overline{N(v)})$\textbackslash $S$

\end{enumerate}
Here the solution set $S$ is the union of $A,B,C,$ and $D$.
\begin{lemma}
\label{lem:4.1}
 Let $\Pi$ be the property `$P_3$-free' and $G$ be a graph such that the subgraph complement of $G$ is $P_3$-free. Let $S\subseteq V(G)$ is a valid solution and $G[S]$ be a clique. Let $u, v \in S$ be distinct. Then  
 \begin{enumerate}[(a)]
     \item $A, C, D, H$ are empty sets.
     \item $G[B]$ is a clique.
 \end{enumerate}
 
\end{lemma}


\begin{proof}
\begin{enumerate}[(a)]
    \item  Here $G[S]$ is a clique and $A$ is in the common non-neighborhood of $u$ and $v$. Moreover, $A\in S$. That implies $A$ must be empty. In $S$, $C$ is in the neighborhood of $u$ but in the non-neighborhood of $v$. So $C$ must be empty. Similarly, $D$ must be empty. Consider a vertex $h\in H$. We know $H$ is not a part of $S$ and $H$ is in the common neighborhood of $u$ and $v$. So $u-h-v$ will be an induced $P_3$ after subgraph complementation. That means $H$ must be empty.
    \item We notice that $B$ is a part of common neighborhood of $u$ and $v$. Moreover, $B\in S$. So $G[B]$ is a clique. 
\end{enumerate}

\end{proof}


\begin{lemma}
\label{lem:4.2}
 Let $\Pi$ be the property `$P_3$-free' and $G$ be a graph such the subgraph complement of $G$ is $P_3$-free. Let $S\subseteq V(G)$ is a valid solution and $G[S]$ be not a clique, and let $u,v\in S$ be distinct vertices such that $uv\notin E(G)$. Then
 \begin{enumerate}[(a)]
\item $C,D,E,F$ are empty sets.
\item $G[A]$ is an independent set.
\item $G[H]$ is a Clique.
\item $A$ and $J$, $J$ and $H$, $B$ and $H$ are disconnected.
\item $A$ and $B$, and $A$ and $H$ are all connected.
 \end{enumerate}
\end{lemma}

\begin{proof}
\begin{enumerate}[(a)]

    \item Consider $c\in C$. Now $C\in (N(u)$\textbackslash $N(v))$ and $C\in S$. So $u-v-c$ will be an induced $P_3$ after subgraph complementation. Therefore, $C$ must be empty. Similarly, $D$ must be empty. Consider $e\in E$. We know $E\in (N(u)$\textbackslash $N(v))$ and $E\notin S$. So $e-u-v$ will be an induced $P_3$ after subgraph complementation. Therefore, $E$ must be empty. Similarly, $F$ must be empty.
    
    \item Consider $a_1$ and $a_2$ in $A$ and $a_{1}a_{2}\in E(G)$. Here $A\in S$ and $A$ is in the non-neighborhood of $u$. So $a_1-u-a_2$ will be an induced $P_3$ after subgraph complementation. Therefore, $G[A]$ must be an independent set.
    
    \item Consider $h_1$ and $h_2$ in $H$ and $h_{1}h_{2}\notin E(G)$. Here $H\in (N(u)$\textbackslash $S$). So $h_{1}-u-h_{2}$ will be an induced $P_3$ after subgraph complementation. Therefore, $G[H]$ must be a Clique.
    
    \item Consider $a\in A$, $j\in J$, and $aj\in E(G)$. Here $A$ is part of $S$ and $J$ is not. Further $A$ and $J$ both are in the non-neighborhood of $u$. So $j,a$, and $u$ will form and induced $P_3$ after subgraph complementation. Therefore, $A$ and $J$ must be disconnected. Now Consider  $j\in J$, $h\in H$, and $jh\in E(G)$. Neither $J$ nor $H$ is a part of $S$. Here $H\in N(u)$ and $j\notin N(u)$. So $j-h-u$ will be an induced $P_3$ after subgraph complementation. Therefore, $J$ and $H$ must be disconnected. Consider $b\in B$, $h\in H$, and $bh\in E(G)$. Here $B\in (N(u)\cap S$) and $H\in (N(u)$\textbackslash $S$). So $b,h$, and $u$ will form and induced $P_3$ after subgraph complementation. Therefore, $B$ and $H$ must be disconnected.
    
    \item Consider $a\in A$, $b\in B$, and $ab\notin E(G)$. Here $B$ is in the neighborhood of $u$ but $A$ is not. Moreover, $A$ and $B$ both belong to $S$. That means, $u, a$, and $b$  will form and induced $P_3$ after subgraph complementation. Therefore, $A$ and $B$ must be all connected. Now consider $a\in A$, $h\in H$, and $ah\notin E(G)$. Here $A$ is in the non-neighborhood of $u$ and $A\in S$. But $H$ is in the neighborhood of $u$ and $H\notin S$. So $h-u-a$ will be an induced $P_3$ after subgraph complementation. Therefore, A and H must be all connected.
\end{enumerate} 
\end{proof}

\begin{theorem}
 For a given graph $G$, finding a solution $S\subseteq V(G)$ such that $G\oplus S$ is `$P_3$-free' can be done in polynomial time.
\end{theorem}

\begin{proof}
Assume that there exists a set $S\subseteq V(G)$ such that $G\oplus S$ is $P_3$-free. Clearly $|S|\geq 2$. The proof is divided into two cases.
\begin{enumerate}[\textbf(1)]
    \item \textbf{When $G[S]$ is a clique :}  Consider any two adjacent vertices $u,v \in S$. In Lemma \ref{lem:4.1} we have proved that $H$ is empty. That means $N(u)\cap N(v)$ consists of $B$ only. From this Lemma, we also know that $A$ is empty. If $G[B]$ is a clique, check $S=\{\{u,v\}\cup B\}$ is a solution or not. If $B$ is empty check, $S=\{u,v\}$ is a solution or not. These steps can be done in polynomial time.
    
    \item \textbf{	When $G[S]$ is not a clique:} Consider any two non-adjacent vertices $u,v \in S$. We notice that $\overline{G[S]}$ should be $P_3$-free. Which means $\overline{G[S]}$ is a cluster. So ${G[S]}$ is a complete multipartite. This implies $G[B]$ is a complete multipartite.  Find all the isolated vertex in $G[A\cup J]$ which are adjacent to all the vertices in $G[B\cup H]$. Let the total number of such vertices be $n$. From Lemma \ref{lem:4.2}(a), we know that $C,D,E,F$ are empty sets. So all of these vertices are equivalent. \textcolor{red}{(We know $J$ and $H$ are disconnected. So if $H$ is not empty, then all of these vertices belong to $A$ )}.Take any $i(0\leq i\leq n )$ vertices from these $n$ vertices and form the set $I_i$. There will be $n$ such non-empty sets. Here $I_0$ denotes the empty set. Now we will consider different sub-cases.
    
    \begin{enumerate}[(2a)]
        \item \textbf{If $G[B\cup H]=I$ is an independent set and $|V(I)|\geq 2$:} From Lemma \ref{lem:4.2}(c) we know that $G[H]$ is a clique. Suppose $|V(I)|=m$. Choose $(m-1)$ vertices out of these $m$ vertices. Let $X$ be the set containing these $m-1$ vertices. There will be total $m$ choices. For each choice check  $S=\{\{u,v\}\cup X \cup I_i\}(0\leq i\leq n )$ is a solution or not. If we consider $H$ to be empty, check $S=\{\{u,v\}\cup I \cup I_i\}(0\leq i\leq n )$ is a solution or not. These steps can be done in polynomial time. \textcolor{red}{(In the first step, $H$ is not empty. So $A=I_{n}$. So here Instead of $I_i$, in S we should include only $I_0$ and $I_n$ }) 
        
        \item \textbf{If $G[B\cup H]$ is a clique:} Let $K$ be the clique. Consider $K=G[B]$ and check $S=\{\{u,v\}\cup V(K) \cup I_i\}(0\leq i\leq n )$ is a solution or not. Now consider $K=G[H]$ and check $S=\{\{u,v\}\cup I_i\}(0\leq i\leq n )$ is a solution or not. These steps can be completed in polynomial time. \textcolor{red}{(In the second step, $H$ is not empty. So $A=I_{n}$. So here Instead of $I_i$, in S we should include only $I_0$ and $I_n$ }) 
        
        \item \textbf{If $G[B\cup H]$ has two connected components and both are cliques:} Let the cliques be $K$ and $L$. First, consider $K$ to be $G[B]$. Check  $S=\{\{u,v\}\cup V(K) \cup I_i\}(0\leq i\leq n )$ is a solution or not. Now consider $L$ to be $G[B]$. Now check $S=\{\{u,v\}\cup V(L) \cup I_i\}(0\leq i\leq n )$ is a solution or not. These steps can be done in polynomial time. \textcolor{red}{(Here $H$ is not empty. So $A=I_{n}$. So here Instead of $I_i$, in S, we should include only $I_0$ and $I_n$ })
        
        \item\textbf{If $G[B\cup H]$ has two connected components, one is a clique and the other is a complete multipartite (but neither a clique nor an independent set:)} From Lemma \ref{lem:4.2}(c) and (d) we observe that  the component which is complete multipartite is $G[B]$. Check $S=\{\{u,v\}\cup V(B)\cup I_i\}(0\leq i\leq n )$ is a solution or not. These steps can be completed in polynomial time. \textcolor{red}{(Here $H$ is not empty. So $A=I_{n}$. So here Instead of $I_i$, in S we should include only $I_0$ and $I_n$ })
        
        \item \textbf{If $G[B\cup H]$ has more than one connected component such that one connected component is a clique (with a number of vertices $\geq 2$) and the other components together form an independent set $I$ such that $|V(I)|\geq 2$:} We know $G[B]$ is a complete multipartite. From Lemma \ref{lem:4.2}(c) and (d) we can conclude That $G[B]=I$. Check $S=\{\{u,v\}\cup I \cup I_i\}(0\leq i\leq n)$ is a solution or not. These steps can be done in polynomial time. \textcolor{red}{(Here $H$ is not empty. So $A=I_{n}$. So here Instead of $I_i$, in S we should include only $I_0$ and $I_n$ })
        
        \item \textbf{If $G[B\cup H]$ is a complete multipartite with no of vertices$\geq 3$ and $G[B\cup H]$ is neither a clique nor an independent set:} In this case $H$ must be empty because $H$ is a clique. So the complete multipartite is $B$. Check $S=\{\{u,v\}\cup V(B)\cup I_i\}(0\leq i\leq n )$ is a solution or not. These steps can be completed in polynomial time.
        
        \item \textbf{If $B\cup H=\emptyset$:} Consider all isolated vertices in $G[A\cup J]$. Let $|V(A\cup J)|=m$. All of these vertices are equivalent. Now take any $i$ ($0\leq i\leq m$) vertices from this set and form the set $P_i$. There will be $m$ such non-empty sets. $P_0$ represents the empty set when $A\cap J$ is empty. Check $S=\{\{u,v\}\cup P_i\}(0\leq i\leq m )$ is a solution or not. These steps can be done in polynomial time. 
        
        
        
        
    \end{enumerate}
    
\end{enumerate}
\end{proof}


\textbf{Class of ${\mathcal{G}^{(1)}}$ and $\overline{\mathcal{G}}^{(1)}$}:
Let $\mathcal{H}_{H}$ be the set of minimal  forbidden subgraphs such that for a given graph $G$, $G\oplus S $ is $H$-free if and only if $G$ does not contain any element of  $\mathcal{H}_{H}$.

\begin{observation}
 The element of $\mathcal{H}_{K_{1}}$ is $K_{1}$. The elements of $\mathcal{H}_{K_{2}}$ are $2K_{2}$ and $P_{3}$. The elements of $\mathcal{H}_{2K_{1}}$ are $C_{4}$ and $\overline{P_{3}}$.
\end{observation}

\begin{lemma}
\label{lem:GS}
   Let $G$ be a graph and $S\subseteq V(G)$. Then $G\oplus S$ = $\overline{\overline{G}\oplus S }$
\end{lemma} 

\begin{proof}
After $G\oplus S$, $G[S]$ becomes $\overline{G[S]}$, $G[G\backslash S]$ remains the same and the adjacencies between the vertices of $G[S]$ and $G[G\backslash S]$ also remain the same.

In $\overline{\overline{G}\oplus S }$, $G[S]$ gets complemented three times. So $G[S]$ becomes $\overline{G[S]}$. But $G[G\backslash S]$ gets complemented two times. So it remains the same. The adjacencies between the vertices of $G[S]$ and $G[G\backslash S]$ gets complemented two times. So the adjacencies remain unaffected. Therefore, we can conclude that $G\oplus S$ = $\overline{\overline{G}\oplus S }$.
\end{proof}

\begin{lemma}
\label{lem:FH}
    For every graph $F$ it holds that $F\in \mathcal{H}_{H}$ if and only if $\overline{F}\in{\mathcal{H}}_{\overline H }$. In other words ${\mathcal{H}}_{ H }$= $\overline{\mathcal{H}}_{\overline H }$ . 
\end{lemma}

\begin{proof}
     Let us assume that $F\in \mathcal{H}_{H}$ and $\overline{F}\notin{\mathcal{H}}_{\overline H }$. This means that $\overline{F}$ is either not forbidden or forbidden but not minimal with respect to subgraph complementation to $ \overline{H}$-free graphs. In the first case, i.e. $\overline{F}$ is not forbidden, it means there exists $S\subseteq V(\overline{F})$ such that $\overline{F}\oplus S$ is free from $\overline{H}$. In other words, $\overline{\overline{F}\oplus S}$ is free from $H$. From Lemma \ref{lem:GS}, it can be said that $F\oplus S$ is free from $H$. So $F$ is not forbidden, which is a contradiction.
     
     In the latter case, $\overline{F}$ is forbidden but not minimal. So there exists an induced subgraph $\overline{F_{1}}$ of $\overline{F}$ which is minimal and forbidden. So there exists no $S\subseteq V{(\overline{F_{1}})}$ such that $\overline{F_{1}}\oplus S$ is free from $\overline{H}$ or $\overline{\overline{F_{1}}\oplus S}$ is free from $H$. From Lemma \ref{lem:GS}, we can say that there exists no $S\subseteq V(F_{1})$ such that $F_{1}\oplus S$ is free from $H$. But $F_{1}$ is an induced subgraph of $F$. So, $F$ is not minimal, which is a contradiction.
 
            Since $\overline{\overline{F}}=F$, the reverse direction is also correct.
\end{proof}
Let $\mathcal{G}^{(1)}$ denote a class of graphs such that its members can be subgraph complemented to a class of graphs $\mathcal{G}$. Let $\overline{\mathcal{G}}$ denote the class of complement graphs of $\mathcal{G}$.
\begin{lemma}
\label{lem:G,G-complement}
$\overline{\mathcal{G}^{(1)}} = \overline{\mathcal{G}}^{(1)}$
\end{lemma}

\begin{proof}
 Let $G$ be a graph such that $G \in \overline{\mathcal{G}}^{(1)}$. So there exists a set $S\subseteq V(G)$ such that $G\oplus S\in \overline{\mathcal{G}}$ or $\overline{\overline{G}\oplus S }\in \overline{\mathcal{G}}$ (from Lemma \ref{lem:GS}). Therefore, $\overline{G}\oplus S \in \mathcal{G}$ or $\overline{G}\in \mathcal{G}^{(1)}$. This implies $G \in \overline{\mathcal{G}^{(1)}}$. Therefore, $\overline{\mathcal{G}}^{(1)}\subseteq\overline{\mathcal{G}^{(1)}}$.\\\\
 Now let  $G \in \overline{\mathcal{G}^{(1)}}$. Then $\overline{G}\in \mathcal{G}^{(1)}$ which means there exist a set $S\subseteq V(\overline{G})$ such that $\overline{G}\oplus S \in \mathcal{G}$. Then $\overline{\overline{G}\oplus S }\in \overline{\mathcal{G}}$. So $G\oplus S\in \overline{\mathcal{G}}$ (from Lemma \ref{lem:GS}). This implies $G\in \overline{\mathcal{G}}^{(1)}$. Therefore, $\overline{\mathcal{G}^{(1)}}\subseteq\overline{\mathcal{G}}^{(1)}$. Earlier we proved that $\overline{\mathcal{G}}^{(1)}\subseteq\overline{\mathcal{G}^{(1)}}$. Therefore, $\overline{\mathcal{G}^{(1)}} = \overline{\mathcal{G}}^{(1)}$.
\end{proof}


\begin{theorem}
Suppose ${\mathcal{G}^{(1)}}$ can be recognised in polynomial time. Then  $\overline{\mathcal{G}}^{(1)}$ can also be recognizable in polynomial time. 
\end{theorem}


\begin{proof}
Let $G$ be a graph and there exist a set $S\subseteq V(G)$ such that $G\oplus S \in \mathcal{G}$.  Let us also assume that we can recognize $\mathcal{G}^{(1)}$ in polynomial time. We need to check whether we can recognize $\overline{\mathcal{G}}^{(1)}$ in polynomial time. We know that, $\overline{\overline{G}\oplus S }$= $G\oplus S$.  Thus, if $\mathcal{G}^{(1)}$ can be subgraph complemented to $\mathcal{G}$ then  $\overline{\mathcal{G}}^{(1)}$ can be subgraph complemented to $\overline{\mathcal{G}}$.  Once we recognize $\mathcal{G}^{(1)}$ in polynomial time, taking complement of $\mathcal{G}^{(1)}$ leads to $\overline{\mathcal{G}^{(1)}}$. From Lemma \ref{lem:GS} we know that $\overline{\mathcal{G}^{(1)}} = \overline{\mathcal{G}}^{(1)}$. Therefore, we can recognize $\overline{\mathcal{G}}^{(1)}$ in polynomial time.  
\end{proof}





\textbf{Other Results:}

\begin{lemma}
 For any graph $H$, there always exist a graph $G$ for which there exists no $S\subseteq V(G)$ such that $G\oplus S$ is $H$-free. The graph $G$ can be constructed as following:
 \begin{itemize}
     \item Let $V(H)=n$. The graph $G$ consists of $n$ copies ($H_1, H_2, \ldots , H_n$) of $H$. So $|V(G)|=n^{2}$.
     \item Take any vertex from $H_1$, any vertex from $H_2$, $\ldots$ , any vertex from $H_n$. Construct $\bar{H}$ using these $n$ vertices.
     \item If the selected vertex in $H_i$  is adjacent to the selected vertex in $H_j$ ($i\neq j$ and $1\leq i,j\leq n$), then make every vertex in $H_i$ adjacent to every vertex in $H_j$. Otherwise keep these two copies disconnected.
 \end{itemize}
\end{lemma}

\begin{proof}
  Assume that there exists $S\subseteq V(G)$ such that $G\oplus S$ is $H$-free. Since the $i^{\text{th}}$ copy induces $H$ in $G$, at least two vertices from $H_i$ must be in $S$. Now consider one vertex each from $H_1\cap S$, $H_2\cap S$, $\ldots$ ,  $H_n\cap S$. These vertices induces $H$ in $G\oplus S$. Hence a contradiction.
\end{proof}

\textbf{SC to Paw-free}



Let $\Pi$ be the property that a given graph $G$ is Paw-free, i.e., no induced subgraph of $G$ forms a Paw. Here we try to find a solution(if exists) $S\subseteq V(G)$ such that $G\oplus S$ is $P_3$-free in polynomial time. Consider $|V(G)|\geq 3$. let $u$ and $v$ be two distinct vertices in $G$. Now depending on the adjacencies of $u$ and $v$ we divide the vertex set of $G$ into eight parts.
\begin{enumerate}[(1)]
	
	\item$A=S\cap \overline {N(u)} \cap \overline{N(v)}$ :- The common non-neighborhood of $u$ and $v$ that belongs to $S$.
	\item $J=(\overline{N(u)}\cap\overline{N(v)})$\textbackslash $S $:-  The common non-neighborhood of $u$ and $v$ in $G$\textbackslash $S$.
	\item $B=S\cap N(u) \cap N(v)$ :- The common neighborhood of $u$ and $v$ that belongs to $S$.
	\item $H=(N(u)\cap N(v))$\textbackslash $S$ :- The common neighborhood of $u$ and $v$ in $G$\textbackslash $S$.
	\item $C=S\cap (N(u)$\textbackslash $N(v))$ :- In $S$, The neighborhood of $u$ but the non-neigborhood of $v$
	\item $E=(N(u)$\textbackslash $N(v))$\textbackslash $S$:- In $G$\textbackslash $S$, the neighborhood of $u$ but the non-neigborhood of $v$
	\item $D=S\cap (N(v)$\textbackslash $N(u))$:-In $S$, the neighborhood of $v$ but the non-neigborhood of $u$
     \item $F=(N(v)$\textbackslash $N(u))$\textbackslash $S$:- In $G$\textbackslash $S$, the neighborhood of $v$ but the non-neigborhood of $u$
	
	

\end{enumerate}
Here the solution set $S$ is the union of $A,B,C,$ and $D$.
\begin{observation}
\label{ob:Paw 1}
 Let $\Pi$ be the property `Paw-free' and $G$ be a graph such that the subgraph complement of $G$ is Paw-free. Let $S\subseteq V(G)$ is a valid solution and $G[S]$ be a clique. Let $u, v \in S$ be distinct. Then  
 \begin{enumerate}[(i)]
    \item $C,D,A$ are empty sets.
    \item $G[B]$ is a clique
    \item $G[H]$ is a complete multipartite.
    \item $H$ and $E$ are disconnected.
 \end{enumerate}
\end{observation}

\begin{proof}
  \begin{enumerate}[(i)]
      \item From the partition, we observe that $C$ is in the non-neighborhood of $v$, and $C\in S$. That implies $C$ must be empty. Similarly, $D$ is empty. We again observe that $A$ is in the common non-neighborhood of $u$ and $v$. Moreover,  $A\in S$ That means $A$ must be empty.
      
      \item We notice that $B$ is a part of common neighborhood of $u$ and $v$. Moreover, $B\in S$. So $G[B]$ is a clique. 
      
      \item Suppose three vertices $h_{1},h_{2},h_{3}$ from $H$ form a $K_{2}\cup K_{1}$. We notice that $H$ is in the common neighborhood of $u$ and $v$ and $h\notin S$. So $h_{1},h_{2},h_{3}$, and $u$ form a Paw after subgraph complementation. Therefore, $H$ must be $K_{2}\cup K_{1}$ free. This implies $G[H]$ is a complete multipartite. 
      
      \item Consider $h\in H$, $e\in E$, and $eh\in E(G)$. So $e,u,h$, and $v$ form a paw after subgraph complementation. Therefore, $E$ and $H$ are disconnected.  
   \end{enumerate}
\end{proof}

\begin{observation}
Let $\Pi$ be the property `Paw-free' and $G$ be a graph such the subgraph complement of $G$ is Paw-free. Let $S\subseteq V(G)$ is a valid solution and $G[S]$ be not a clique, and let $u,v\in S$ be distinct vertices such that $uv\notin E(G)$. Then
\begin{enumerate}[(i)]
    \item $C$, and $D$ are cliques.
    \item $E$, and $F$ are Independent sets.
    \item $G[A]$ is a clique.
    \item $G[H]$ is a complete multipartite.
    \item $A$ and $J$, $H$ and $J$, $B$ and $H$, $A$ and $C$, $A$ and $D$ are nonadjacent.
    \item $A$ and $E$, $A$ and $B$, $H$ and $E$, $H$ and $C$,$H$ and $D$ are all adjacent. 
\end{enumerate}
\end{observation}
\begin{proof}
  \begin{enumerate}[(i)]
      \item Consider $c_{1},c_{2}\in C$, and $c_{1}c_{2}\notin E(G)$. Then $c_{1},c_{2},v$, and $u$ form a Paw after subgraph complementation. Therefore, $C$ must be a clique. Similarly, $D$ is a clique.
      
      \item Consider $e_{1},e_{2}\in E$, and $e_{1}e_{2}\in E(G)$. Then $e_{1},e_{2},u$, and $v$ form a Paw after subgraph complementation. Therefore, $E$ must be an independent set. Similarly, $F$ is an independent set.
      
      \item Consider three vertices $a_{1}, a_{2}$, and  $a_{3}$ from $A$. Suppose they form an induced $P_3$. Then $a_{1}, a_{2}, a_{3}$, and $u$ from a Paw after partial complementation. So $A$ should be $P_{3}$-free. That means $A$ is a cluster.
      
      \item Consider three vertices $h_{1}, h_{2}$, and  $h_{3}$ from $H$. Suppose they form an induced $K_{2}\cup K_{1}$. Then $h_{1}, ah{2}, h_{3}$, and $u$ from a Paw after partial complementation. So $H$ should be $K_{2}\cup K_{1}$-free. That means $H$ is a complete multipartite.
      
      \item Consider $a\in A$, $j\in J$ and $aj\in E(G)$. Then $u,v,a$, and $j$ form a Paw after subgraph complementation. Therefore, $A$ and $J$ are nonadjacent. Consider $h\in H$, $j\in J$ and $hj\in E(G)$. Then $u,v,h$, and $j$ form a Paw after subgraph complementation. Therefore, $H$ and $J$ are nonadjacent. Consider $b\in B$, $h\in H$ and $bh\in E(G)$. Then $u,v,h$, and $b$ form a Paw after subgraph complementation. Therefore, $B$ and $H$ are nonadjacent. Consider $a\in A$, $c\in C$ and $ac\in E(G)$. Then $a,u,v$, and $c$ form a Paw after subgraph complementation. Therefore, $A$ and $C$ are nonadjacent. Similarly, $A$ and $D$ are nonadjacent.
     
     \item Consider $a\in A$, $e\in E$ and $ae\notin E(G)$. Then $a,v,u$, and $e$ form a Paw after subgraph complementation. Therefore, $A$ and $E$ should be all adjacent. Consider $a\in A$, $b\in B$ and $ab\notin E(G)$. Then $u,v,a$, and $b$ form a Paw after subgraph complementation. Therefore, $A$ and $B$ should be all adjacent. Consider $h\in H$, $e\in E$ and $he\notin E(G)$. Then $h,v,u$, and $e$ form a Paw after subgraph complementation. Therefore, $H$ and $E$ should be all adjacent. Consider $h\in H$, $c\in C$ and $hc\notin E(G)$. Then $h,u,v$, and $c$ form a Paw after subgraph complementation. Therefore, $H$ and $C$ should be all adjacent. Similarly,  $H$ and $D$ are adjacent.

    \end{enumerate}
\end{proof}

\begin{observation}
If $H$ is non-empty, Then
\begin{enumerate}[(i)]
    \item $J$ and $C$, $J$ and $D$, $B$ and $E$  are nonadjacent.
    \item $B$ and $C$, $B$ and $D$, $C$ and $E$, $D$ and $F$ are all adjacent.
\end{enumerate}
\end{observation}

\begin{proof}
  \begin{enumerate}[(i)]
      \item 
  \end{enumerate}
\end{proof}

\begin{enumerate}[(i)]
	\item $S_{uv}=S\cap N(u) \cap N(v)$ :- In $S$, the common neighborhood of $u$ and $v$.
	\item$S_{\overline{uv}}=S\cap \overline {N(u)} \cap \overline{N(v)}$ :- In $S$, the common non-neighborhood of $u$ and $v$.
	
	\item $S_{u\overline{v}}=S\cap (N(u)$\textbackslash $N(v))$ :- In $S$, the neighborhood of $u$ but the non-neigborhood of $v$.
	\item $S_{\overline{u}v}=S\cap (N(v)$\textbackslash $N(u))$ :-In $S$, the neighborhood of $v$ but the non-neigborhood of $u$.

	\item $T_{uv}=(N(u)\cap N(v))$\textbackslash $S$ :- In $G$\textbackslash $S$, the common neighborhood of $u$ and $v$ in $G$\textbackslash $S$.
     \item $T_{\overline{uv}}=(\overline{N(u)}\cap\overline{N(v)})$\textbackslash $S $ :- In $S$, the common non-neighborhood of $u$ and $v$ in $G$\textbackslash $S$.
	\item $T_{u\overline{v}}=(N(u)$\textbackslash $N(v))$\textbackslash $S$ :- In $G$\textbackslash $S$, the neighborhood of $u$ but the non-neigborhood of $v$.
	
     \item $T_{\overline{u}v}=(N(v)$\textbackslash $N(u))$\textbackslash $S$ :- In $G$\textbackslash $S$, the neighborhood of $v$ but the non-neigborhood of $u$.
\end{enumerate}


    


==> conclusion.tex <==
\section{Concluding Remarks}


==> figs/inductive/k6.tex <==
\begin{tikzpicture}[myv/.style={circle, draw, inner sep=0.5pt}, myv1/.style={circle, draw, inner sep=1pt,fill=black},myv2/.style={rectangle,color=white, draw,inner sep=1.5pt}, myv3/.style={rectangle,color=white, draw, inner sep=1.5pt}]
  \node (z) at (0,0) {};

  \node[myv] (a) at (90:0.25) {};
  \node[myv] (b) at (150:0.25) {};
  \node[myv] (c) at (210:0.25) {};
  \node[myv] (d) at (270:0.25) {};
  \node[myv] (e) at (330:0.25) {};
  \node[myv] (f) at (30:0.25) {};
 % \node[myv1] (g) at (30:0.5) {};%4
 % \node[myv1] (h) at (65:0.5) {};%6

% \node[myv2][fit=(a) (d)]{}; 
  %\node[myv3][fit=(e) (h)]{}; 

  \draw (a) -- (b); 
  \draw (a) -- (c);
  \draw (a) -- (d);
  \draw (a) -- (e);
  \draw (a) -- (f);
%  \draw (a) -- (g);
 % \draw (a) -- (h);
  \draw (b) -- (c);
  \draw (b) -- (d);
  \draw (b) -- (e);
  \draw (b) -- (f);
% \draw (b) -- (g);
%  \draw (b) -- (h);
  \draw (c) -- (d);
  \draw (c) -- (e);
  \draw (c) -- (f);
 % \draw (c) -- (g);
  %\draw (c) -- (h);
  \draw (d) -- (e);
 \draw (d) -- (f);
 % \draw (d) -- (g);
 % \draw (d) -- (h);
  \draw (e) -- (f);
  %\draw (e) -- (g);
 % \draw (e) -- (h);
 % \draw (f) -- (g);
 % \draw (f) -- (h);
 % \draw (g) -- (h);
\end{tikzpicture}


